Uncertainty quantification for damage mechanics models using the bootstrap method

We quantify the uncertainty of the L\"ammer model of damage evolution when fitted to (noisy) observations of damage evolution in cyclic fatigue experiments with and without dwell time. We therefore develop a bootstrap method by sampling over blocks of load cycles in the experiments in order to quantify the uncertainty in the material parameters of the L\"ammer damage evolution equation. We first develop a resilient optimization algorithm for parameter identification based on numerical solutions of damage evolution. The uncertainty is quantified on three levels: distribution of parameters of the L\"ammer model, confidence bands for the solutions of damage evolution, and distributions of failure times. The method is tested on several data sets, committing considerable high-performance computing resources to the task.

==> sage_style_guide_template.tex <==

% \section{Introduction}
% Many authors submitting to research journals use \LaTeXe\ to
% prepare their papers. This paper describes the
% \textsf{\journalclass} class file which can be used to convert
% articles produced with other \LaTeXe\ class files into the correct
% form for submission to \textit{SAGE Publications}.

% The \textsf{\journalclass} class file preserves much of the
% standard \LaTeXe\ interface so that any document which was
% produced using the standard \LaTeXe\ \textsf{article} style can
% easily be converted to work with the \textsf{\journalclassshort}
% style. However, the width of text and typesize will vary from that
% of \textsf{article.cls}; therefore, \textit{line breaks will change}
% and it is likely that displayed mathematics and tabular material
% will need re-setting.

% In the following sections we describe how to lay out your code to
% use \textsf{\journalclass} to reproduce much of the typographical look of
% the \textit{SAGE} journal that you wish to submit to. However, this paper is not a guide to
% using \LaTeXe\ and we would refer you to any of the many books
% available (see, for example, \cite{R1}, \cite{R2} and \cite{R3}).

% \section{The three golden rules}
% Before we proceed, we would like to stress \textit{three golden
% rules} that need to be followed to enable the most efficient use
% of your code at the typesetting stage:
% \begin{enumerate}
% \item[(i)] keep your own macros to an absolute minimum;

% \item[(ii)] as \TeX\ is designed to make sensible spacing
% decisions by itself, do \textit{not} use explicit horizontal or
% vertical spacing commands, except in a few accepted (mostly
% mathematical) situations, such as \verb"\," before a
% differential~d, or \verb"\quad" to separate an equation from its
% qualifier;

% \item[(iii)] follow the journal reference style.
% \end{enumerate}

% \section{Getting started} The \textsf{\journalclassshort} class file should run
% on any standard \LaTeXe\ installation. If any of the fonts, style
% files or packages it requires are missing from your installation,
% they can be found on the \textit{\TeX\ Collection} DVDs or downloaded from
% CTAN.

% \begin{figure*}
% \setlength{\fboxsep}{0pt}%
% \setlength{\fboxrule}{0pt}%
% \begin{center}
% \begin{boxedverbatim}
% \documentclass[<options>]{sagej}

% \begin{document}

% \runninghead{<Author surnames>}

% \title{<Initial capital only>}

% \author{<An Author\affilnum{1},
% Someone Else\affilnum{2} and
% Perhaps Another\affilnum{1}>}

% \affiliation{<\affilnum{1}First and third authors' affiliation\\
% \affilnum{2}Second author affiliation>}

% \corrauth{<Corresponding author's name and full postal address>}

% \email{<Corresponding author's email address>}

% \begin{abstract}
% <Text>
% \end{abstract}

% \keywords{<List keywords>}

% \maketitle

% \section{Introduction}
% .
% .
% .
% \end{boxedverbatim}
% \end{center}
% \caption{Example header text.\label{F1}}
% \end{figure*}

% \section{The article header information}
% The heading for any file using \textsf{\journalclass} is shown in
% Figure~\ref{F1}. You must select options for the trim/text area and
% the reference style of the journal you are submitting to.
% The choice of \verb+options+ are listed in Table~\ref{T1}.

% \begin{table}[h]
% \small\sf\centering
% \caption{The choice of options.\label{T1}}
% \begin{tabular}{lll}
% \toprule
% Option&Trim and font size&Columns\\
% \midrule
% \texttt{shortAfour}& 210 $\times$ 280 mm, 10pt& Double column\\
% \texttt{Afour} &210 $\times$ 297 mm, 10pt& Double column\\
% \texttt{MCfour} &189 $\times$ 246 mm, 10pt& Double column\\
% \texttt{PCfour} &170 $\times$ 242 mm, 10pt& Double column\\
% \texttt{Royal} &156 $\times$ 234 mm, 10pt& Single column\\
% \texttt{Crown} &7.25 $\times$ 9.5 in, 10pt&Single column\\
% \texttt{Review} & 156 $\times$ 234 mm, 12pt & Single column\\
% \bottomrule
% \end{tabular}\\[10pt]
% \begin{tabular}{ll}
% \toprule
% Option&Reference style\\
% \midrule
% \texttt{sageh}&SAGE Harvard style (author-year)\\
% \texttt{sagev}&SAGE Vancouver style (superscript numbers)\\
% \texttt{sageapa}&APA style (author-year)\\
% \bottomrule
% \end{tabular}
% \end{table}

% For example, if your journal is short A4 sized, uses Times fonts and has Harvard style references then you would need\\
% {\small\verb+\documentclass[ShortAfour,times,sageh]{sagej}+}

% Most \textit{SAGE} journals are published using Times fonts but if for any reason you have a problem using Times you can
% easily resort to Computer Modern fonts by removing the
% \verb"times" option.

% \subsection{`Review' option}
% Some journals (for example, \emph{Journal of the Society for Clinical Trials}) require that
% papers are set single column and with a larger font size to help with the review process.
% If this is a requirement for the journal that you are submitting to, just add the \verb+Review+ option to the \verb+\documenclass[]{sagej}+ line.

% \subsection{Remarks}
% \begin{enumerate}
% \item[(i)] In \verb"\runninghead" use `\textit{et~al.}' if there
% are three or more authors.

% \item[(ii)] For multiple author papers please note the use of \verb"\affilnum" to
% link names and affiliations. The corresponding author details need to be included using the
% \verb+\corrauth+ and \verb+\email+ commands.

% \item[(iii)] For submitting a double-spaced manuscript, add
% \verb"doublespace" as an option to the documentclass line.

% \item[(iv)] The abstract should be capable of standing by itself,
% in the absence of the body of the article and of the bibliography.
% Therefore, it must not contain any reference citations.

% \item[(v)] Keywords are separated by commas.

% \item[(vi)] If you are submitting to a \textit{SAGE} journal that requires numbered sections (for example, IJRR), please add the command
%   \verb+\setcounter{secnumdepth}{3}+ just above the \verb+\begin{document}+ line.

% \end{enumerate}


% \section{The body of the article}

% \subsection{Mathematics} \textsf{\journalclass} makes the full
% functionality of \AmS\/\TeX\ available. We encourage the use of
% the \verb"align", \verb"gather" and \verb"multline" environments
% for displayed mathematics. \textsf{amsthm} is used for setting
% theorem-like and proof environments. The usual \verb"\newtheorem"
% command needs to be used to set up the environments for your
% particular document.

% \subsection{Figures and tables} \textsf{\journalclass} includes the
% \textsf{graphicx} package for handling figures.

% Figures are called in as follows:
% \begin{verbatim}
% \begin{figure}
% \centering
% \includegraphics{<figure name>}
% \caption{<Figure caption>}
% \end{figure}
% \end{verbatim}

% For further details on how to size figures, etc., with the
% \textsf{graphicx} package see, for example, \cite{R1}
% or \cite{R3}.

% The standard coding for a table is shown in Figure~\ref{F2}.

% \begin{figure}
% \setlength{\fboxsep}{0pt}%
% \setlength{\fboxrule}{0pt}%
% \begin{center}
% \begin{boxedverbatim}
% \begin{table}
% \small\sf\centering
% \caption{<Table caption.>}
% \begin{tabular}{<table alignment>}
% \toprule
% <column headings>\\
% \midrule
% <table entries
% (separated by & as usual)>\\
% <table entries>\\
% .
% .
% .\\
% \bottomrule
% \end{tabular}
% \end{table}
% \end{boxedverbatim}
% \end{center}
% \caption{Example table layout.\label{F2}}
% \end{figure}

% \subsection{Cross-referencing}
% The use of the \LaTeX\ cross-reference system
% for figures, tables, equations, etc., is encouraged
% (using \verb"\ref{<name>}" and \verb"\label{<name>}").

% \subsection{End of paper special sections}
% Depending on the requirements of the journal that you are submitting to,
% there are macros defined to typeset various special sections.

% The commands available are:
% \begin{verbatim}
% \begin{acks}
% To typeset an
%   "Acknowledgements" section.
% \end{acks}
% \end{verbatim}

% \begin{verbatim}
% \begin{biog}
% To typeset an
%   "Author biography" section.
% \end{biog}
% \end{verbatim}

% \begin{verbatim}
% \begin{biogs}
% To typeset an
%   "Author Biographies" section.
% \end{biogs}
% \end{verbatim}

% %\newpage

% \begin{verbatim}
% \begin{dci}
% To typeset a "Declaration of
%   conflicting interests" section.
% \end{dci}
% \end{verbatim}

% \begin{verbatim}
% \begin{funding}
% To typeset a "Funding" section.
% \end{funding}
% \end{verbatim}

% \begin{verbatim}
% \begin{sm}
% To typeset a
%   "Supplemental material" section.
% \end{sm}
% \end{verbatim}

% \subsection{Endnotes}
% Most \textit{SAGE} journals use endnotes rather than footnotes, so any notes should be coded as \verb+\endnote{<Text>}+.
% Place the command \verb+\theendnotes+ just above the Reference section to typeset the endnotes.

% To avoid any confusion for papers that use Vancouver style references,  footnotes/endnotes should be edited into the text.

% \subsection{References}
% Please note that the files \textsf{SageH.bst} and \textsf{SageV.bst} are included with the class file
% for those authors using \BibTeX.
% The files work in a completely standard way, and you just need to uncomment one of the lines in the below example depending on what style you require:
% \begin{verbatim}
% %%Harvard (name/date)
% %\bibliographystyle{SageH}
% %%Vancouver (numbered)
% %\bibliographystyle{SageV}
% \bibliography{<YourBibfile.bib>}
% \end{verbatim}
% and remember to add the relevant option to the \verb+\documentclass[]{sagej}+ line as listed in Table~\ref{T1}. 

% %\section{Support for \textsf{\journalclass}}
% %We offer on-line support to participating authors. Please contact
% %us via e-mail at \dots
% %
% %We would welcome any feedback, positive or otherwise, on your
% %experiences of using \textsf{\journalclass}.

% \section{Copyright statement}
% Please  be  aware that the use of  this \LaTeXe\ class file is
% governed by the following conditions.

% \subsection{Copyright}
% Copyright \copyright\ \volumeyear\ SAGE Publications Ltd,
% 1 Oliver's Yard, 55 City Road, London, EC1Y~1SP, UK. All
% rights reserved.

% \subsection{Rules of use}
% This class file is made available for use by authors who wish to
% prepare an article for publication in a \textit{SAGE Publications} journal.
% The user may not exploit any
% part of the class file commercially.

% This class file is provided on an \textit{as is}  basis, without
% warranties of any kind, either express or implied, including but
% not limited to warranties of title, or implied  warranties of
% merchantablility or fitness for a particular purpose. There will
% be no duty on the author[s] of the software or SAGE Publications Ltd
% to correct any errors or defects in the software. Any
% statutory  rights you may have remain unaffected by your
% acceptance of these rules of use.

% \begin{acks}
% This class file was developed by Sunrise Setting Ltd,
% Brixham, Devon, UK.\\
% Website: \url{http://www.sunrise-setting.co.uk}
% \end{acks}

% \begin{thebibliography}{99}
% \bibitem[Kopka and Daly(2003)]{R1}
% Kopka~H and Daly~PW (2003) \textit{A Guide to \LaTeX}, 4th~edn.
% Addison-Wesley.

% \bibitem[Lamport(1994)]{R2}
% Lamport~L (1994) \textit{\LaTeX: a Document Preparation System},
% 2nd~edn. Addison-Wesley.

% \bibitem[Mittelbach and Goossens(2004)]{R3}
% Mittelbach~F and Goossens~M (2004) \textit{The \LaTeX\ Companion},
% 2nd~edn. Addison-Wesley.

% \end{thebibliography}

% \end{document}

